Foundation Model-oriented Robustness: Robust Image Model Evaluation with Pretrained Models

Machine learning has demonstrated remarkable performance over finite datasets, yet whether the scores over the fixed benchmarks can sufficiently indicate the model's performance in the real world is still in discussion. In reality, an ideal robust model will probably behave similarly to the oracle (e.g., the human users), thus a good evaluation protocol is probably to evaluate the models' behaviors in comparison to the oracle. In this paper, we introduce a new robustness measurement that directly measures the image classification model's performance compared with a surrogate oracle (i.e., a foundation model). Besides, we design a simple method that can accomplish the evaluation beyond the scope of the benchmarks. Our method extends the image datasets with new samples that are sufficiently perturbed to be distinct from the ones in the original sets, but are still bounded within the same image-label structure the original test image represents, constrained by a foundation model pretrained with a large amount of samples. As a result, our new method will offer us a new way to evaluate the models' robustness performance, free of limitations of fixed benchmarks or constrained perturbations, although scoped by the power of the oracle. In addition to the evaluation results, we also leverage our generated data to understand the behaviors of the model and our new evaluation strategies.

==> secs/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{We will release the code and datasets soon}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:con}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:impact}} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include the code, data, instruction and detailed results in the Supplementary Material.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The training details are included in the Supplementary, as well as the Annotations.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{The standard error bars could be found in the Supplementary}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We include the resources in Section~\ref{sec:setup}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include in the Supplementary Material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> secs/impact.tex <==
The primary goal of this paper is to introduce a new evaluation protocol for vision machine learning research that can generate sufficiently perturbed samples from the original samples while maintaining the image-label structures by assuming an oracle. Thus, we can introduce significant variations of the existing data while being free from additional human efforts. With our approach, we hope to renew the benchmarks for current robustness evaluation, offer understandings of the behaviors of deep vision models and potentially facilitate the generation of more truly robust models. Increasing the robustness of vision models can enhance their reliability and safety, which leads to the trustworthy artificial intelligence and contributes to a wide range of application scenarios (\textit{e.g.,} manufacturing automation, surveillance systems, \textit{etc.}). Manufacturing automation can improve the production efficiency, but may also trigger social issues related to job looses and industrial restructuring. Advanced surveillance systems 
are conducive to improving social security, but may also raise public concerns about personal privacy violations.

We encourage further work to understand the limitations of machine vision models in OOD settings. More robust models carry the potential risk of automation bias, i.e., an undue trust in vision models. However, even if models are robust against corruptions in finite OOD datasets, they might still quickly fail on the massive generic perturbations existing in the real-world data space, \textit{i.e.,} the perturbations offered by our approach. Understanding under what conditions model decisions can be deemed reliable or not is still an open research question that deserves further attention.

==> secs/related.tex <==
Before we conclude, 
we devote a section to other related works of our contribution, 
especially the works on different strategies of generating counterfactual images, 
though these works do not usually contribute as a protocol to evaluate the robustness of models, 
but to explain the model's decisions. 

To explain model's decisions, 
the generated counterfactual images \citep{wachter2017counterfactual}
are usually expected to differ from the original images 
through a minimum set of image features (\textit{i.e.}, sparse)
while maintaining the causality structure (\textit{i.e.}, proximal) 
and altering the model's decision (\textit{i.e.}, valid),
as described by \citep{dhurandhar2018explanations,russell2019efficient,mothilal2020explaining,looveren2021interpretable}. 

Most of these methods 
builds upon a conditional GAN structure \citep{joshi2018xgems,liu2019generative,sauer2021counterfactual,van2021conditional,yang2021generative}
or generative model structure \citep{denton2019detecting,singla2019explanation,rodriguez2021beyond}.

While these methods introduce different techniques and assumptions to maintain the underlying causal structure of the generated images, 
\citet{mahajan2019preserving} showed that 
this goal cannot be fulfilled, in general, with statistical techniques alone:
extra knowledge about underlying causal structure is needed. 

From method perspective, 
the key differences between our contributions 
and these works
lie in two folds: 
we free the need of the underlying causal structure 
(although introducing the dependence on plausible oracle); 
we do not limit the perturbation to be sparse 
to fully test the model's robustness against a wide range of perturbations. 



